Log-Riemann Surfaces

We introduce the notion of log-Riemann surfaces. These are Riemann surfaces given by cutting and pasting planes together isometrically, and come equipped with a holomorphic local diffeomorphism to C called the projection map, and a corresponding flat metric obtained by pulling back the Euclidean metric. We define ramification points to be the points added in the metric completion of the surface with respect to the induced path metric; any such point has a well-defined order $1 \leq n \leq +\infty$ such that the projection map restricted to a small punctured neighbourhood of the point is an $n-to-1$ covering of a punctured disk in C. We prove that simply connected log-Riemann surfaces with finitely many ramification points are biholomorphic to C and the uniformization, with respect to the distinguished charts on the surface given by the projection map, is given by an entire function of the form $F(z) = \int Q(z)e^{P(z)} dz$ where $P, Q$ are polynomials of degrees equal to the number of infinite and finite order ramification points respectively. We also develop an algebraic theory for such log-Riemann surfaces, defining a ring of functions on the surface with finite values at all ramification points, such that the ring separates all points including the infinite order ramification points.

==> figures/I4fig1 <==
#FIG 3.2
Portrait
Center
Metric
A4 
100.0
Single
-2
1200 2
3 0 0 1 0 0 100 1 -1  6.40 0 0 0 3
       3600 6570 3240 6660 2970 6660
       0.0000 1.0000 0.0000
3 0 0 1 0 0 100 1 -1  6.40 0 0 0 3
       4590 5850 4320 5940 3240 5940
       0.0000 1.0000 0.0000
3 0 0 1 0 0 100 1 -1  6.40 0 0 0 3
       5400 4950 4500 5220 1890 4950
       0.0000 1.0000 0.0000
3 0 0 1 0 0 100 1 -1  6.40 0 0 0 3
       5850 4050 5400 4320 2340 4320
       0.0000 1.0000 0.0000
3 0 0 1 0 0 100 1 -1  6.40 0 0 0 3
       6210 3150 5760 3420 2700 3510
       0.0000 1.0000 0.0000
3 0 0 1 0 0 100 1 -1  6.40 0 0 0 3
       6210 2250 5760 2520 2700 2610
       0.0000 1.0000 0.0000
3 0 0 1 0 0 100 1 -1  6.40 0 0 0 3
       6210 2250 6930 1350 10800 1350
       0.0000 1.0000 0.0000
3 0 0 1 0 0 100 1 -1  6.40 0 0 0 3
       6210 3150 6660 2250 10800 2250
       0.0000 1.0000 0.0000
3 0 0 1 0 0 100 1 -1  6.40 0 0 0 3
       5850 4050 6660 3150 10800 3150
       0.0000 1.0000 0.0000
3 0 0 1 0 0 100 1 -1  6.40 0 0 0 3
       5400 4950 6075 4050 10800 4050
       0.0000 1.0000 0.0000
3 0 0 1 0 0 100 1 -1  6.40 0 0 0 3
       4590 5850 5625 4950 10800 4950
       0.0000 1.0000 0.0000
3 0 0 1 0 0 100 1 -1  6.40 0 0 0 3
       3600 6570 5175 5850 10800 5850
       0.0000 1.0000 0.0000
3 0 0 1 0 0 100 1 -1  6.40 0 0 0 4
       1800 7200 3600 7200 4230 6570 10800 6750
       0.0000 1.0000 1.0000 0.0000
1 1 1 1 0 0 100 1 20  6.40 1 0.0 6750 9000 60 60 6690 8940 6810 9060
2 1 0 1 0 0 100 1 -1  0  0 0 12 0 0 2
       450 9000 10800 9000
2 1 0 1 0 0 100 1 -1  0  0 0 12 1 0 2
  0 0 1.0 144.00 240.00
       6750 7560 6750 8730
1 1 1 1 0 0 100 1 20  6.40 1 0.0 4500 7560 60 60 4440 7500 4560 7620
1 1 1 1 0 0 100 1 20  6.40 1 0.0 4500 7830 60 60 4440 7770 4560 7890
1 1 1 1 0 0 100 1 20  6.40 1 0.0 4500 8100 60 60 4440 8040 4560 8160
6 4560 840 4440 1500
1 1 1 1 0 0 100 1 20  6.40 1 0.0 4500 900 60 60 4440 840 4560 960
1 1 1 1 0 0 100 1 20  6.40 1 0.0 4500 1170 60 60 4440 1110 4560 1230
1 1 1 1 0 0 100 1 20  6.40 1 0.0 4500 1440 60 60 4440 1380 4560 1500
-6
1 1 1 1 0 0 100 1 20  6.40 1 0.0 2790 8280 0 0 2790 8280 2790 8280
2 1 1 1 0 0 100 1 -1  6.40 0 0 12 0 0 2
       6750 900 6750 7470
3 0 0 1 0 0 100 1 -1  0  0 0 0 4
       450 2700 900 4500 1170 6300 10800 6300
       0.0000 1.0000 1.0000 0.0000
3 0 0 1 0 0 100 1 -1  0  0 0 0 4
       450 1800 900 4500 1350 7200 10800 7200
       0.0000 1.0000 1.0000 0.0000
3 0 0 1 0 0 100 1 -1  0  0 0 0 4
       450 7200 900 4500 1350 1800 10800 1800
       0.0000 1.0000 1.0000 0.0000
3 0 0 1 0 0 100 1 -1  0  0 0 0 4
       450 6300 900 4500 1170 2700 10800 2700
       0.0000 1.0000 1.0000 0.0000
3 0 0 1 0 0 100 1 -1  0  0 0 0 4
       450 3600 900 4500 1170 5400 10800 5400
       0.0000 1.0000 1.0000 0.0000
3 0 0 1 0 0 100 1 -1  0  0 0 0 4
       450 5400 900 4500 1170 3600 10800 3600
       0.0000 1.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  0  0 0 12 0 0 2
       450 4500 10800 4500
4 0 0 100 1 32 22.0 0.0 4 448.0 192.0 7020 8190 p\001
4 0 0 100 1 0 16.0 0.0 4 336.0 128.0 6930 9540 1\001
4 0 0 100 1 0 22.0 0.0 4 448.0 144.0 6750 9450 z\001


==> figures/i1example3 <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
6 4410 1620 7875 2835
2 3 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 5
	 7335 2790 4455 2790 4950 1665 7830 1665 7335 2790
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6165 2205 7560 2250
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6210 2205 7605 2160
4 0 0 50 0 0 18 0.0000 4 180 135 6030 2160 0\001
-6
6 4410 2925 7875 4140
2 3 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 5
	 7335 4095 4455 4095 4950 2970 7830 2970 7335 4095
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6165 3510 7560 3555
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6210 3510 7605 3465
4 0 0 50 0 0 18 0.0000 4 180 135 6030 3465 0\001
-6
6 4410 5265 7875 6480
2 3 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 5
	 7335 6435 4455 6435 4950 5310 7830 5310 7335 6435
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6165 5850 7560 5895
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6210 5850 7605 5805
4 0 0 50 0 0 18 0.0000 4 180 135 6030 5805 0\001
-6
6 2835 3780 3060 4095
4 0 0 50 0 33 30 0.0000 4 285 210 2835 4050 S\001
-6
1 4 0 2 0 0 50 0 20 6.000 1 0.0000 6052 4297 32 32 6075 4275 6030 4320
1 4 0 2 0 0 50 0 20 6.000 1 0.0000 6030 4590 32 32 6053 4568 6008 4613
1 4 0 2 0 0 50 0 20 6.000 1 0.0000 6030 4905 32 32 6053 4883 6008 4928
1 4 0 2 0 0 50 0 20 0.000 1 0.0000 5670 2205 60 60 5610 2205 5730 2205
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 6255 2385 6435 2520 6255 2610
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 6435 3060 6255 3195 6435 3285
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 6435 1755 6255 1890 6435 1980
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 6435 5400 6255 5535 6435 5625
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 6210 3690 6390 3825 6210 3915
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 6210 6030 6390 6165 6210 6255
3 0 0 2 0 0 50 0 -1 6.000 0 0 0 5
	 5670 2205 5895 2475 6300 2565 6885 2430 7020 2250
	 0.000 1.000 1.000 1.000 0.000
3 0 0 2 0 0 50 0 -1 6.000 0 0 0 5
	 5670 3510 5895 3240 6300 3150 6885 3285 7020 3465
	 0.000 1.000 1.000 1.000 0.000
3 0 0 2 0 0 50 0 -1 6.000 0 0 0 5
	 5670 5850 5895 5580 6300 5490 6885 5625 7020 5805
	 0.000 1.000 1.000 1.000 0.000
3 0 0 2 0 0 50 0 -1 6.000 0 0 0 5
	 5670 5850 5895 6120 6300 6210 6885 6075 7020 5895
	 0.000 1.000 1.000 1.000 0.000
3 0 0 2 0 0 50 0 -1 6.000 0 0 0 5
	 5670 3510 5895 3780 6300 3870 6885 3735 7020 3555
	 0.000 1.000 1.000 1.000 0.000
3 0 0 2 0 0 50 0 -1 6.000 0 0 0 5
	 5670 2205 5895 1935 6300 1845 6885 1980 7020 2160
	 0.000 1.000 1.000 1.000 0.000
4 0 0 50 0 0 80 0.0000 4 1035 570 8055 4725 }\001
4 0 0 50 0 0 20 0.0000 4 270 1005 8640 4545 n planes\001
4 0 0 50 0 0 20 0.0000 4 210 1785 1665 3690 Surface of the \001
4 0 0 50 0 0 20 0.0000 4 255 1185 1665 4050 nth root,  \001
4 0 0 50 0 0 16 0.0000 4 105 120 3060 4140 n\001


==> figures/i1example7 <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
6 6300 1350 6480 2160
1 3 0 2 0 0 50 0 20 6.000 1 0.0000 6390 2070 45 45 6390 2070 6390 2115
1 3 0 2 0 0 50 0 20 6.000 1 0.0000 6390 1755 45 45 6390 1755 6390 1800
1 3 0 2 0 0 50 0 20 6.000 1 0.0000 6390 1440 45 45 6390 1440 6390 1485
-6
6 6300 6615 6480 7425
1 3 0 2 0 0 50 0 20 6.000 1 0.0000 6390 7335 45 45 6390 7335 6390 7380
1 3 0 2 0 0 50 0 20 6.000 1 0.0000 6390 7020 45 45 6390 7020 6390 7065
1 3 0 2 0 0 50 0 20 6.000 1 0.0000 6390 6705 45 45 6390 6705 6390 6750
-6
6 1620 3645 3555 4455
6 3015 3960 3240 4275
4 0 0 50 0 33 30 0.0000 4 285 210 3015 4230 S\001
-6
4 0 0 50 0 0 20 0.0000 4 270 1425 1620 4230 logarithm,  \001
4 0 0 50 0 0 16 0.0000 4 225 300 3240 4365 log\001
4 0 0 50 0 0 20 0.0000 4 210 1710 1620 3870 Surface of the\001
-6
2 3 0 2 0 7 50 0 -1 6.000 0 0 7 0 0 5
	 7515 3690 4140 3690 5085 2565 8460 2565 7515 3690
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6345 3105 7965 3150
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6345 3119 8010 3060
2 3 0 2 0 7 50 0 -1 6.000 0 0 7 0 0 5
	 7515 5085 4140 5085 5085 3960 8460 3960 7515 5085
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6345 4500 7965 4545
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6345 4514 8010 4455
2 3 0 2 0 7 50 0 -1 6.000 0 0 7 0 0 5
	 7425 6435 4050 6435 4995 5310 8370 5310 7425 6435
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6255 5850 7875 5895
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6255 5864 7920 5805
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 2
	 11250 4185 11115 4365
4 0 0 50 0 0 18 0.0000 4 180 135 6165 3060 0\001
4 0 0 50 0 0 18 0.0000 4 180 135 6165 4455 0\001
4 0 0 50 0 0 18 0.0000 4 180 135 6075 5850 0\001
4 0 0 50 0 0 100 0.0000 4 1290 720 8730 4455 }\001
4 0 0 50 0 0 20 0.0000 4 285 1140 9585 3690 infinitely\001
4 0 0 50 0 0 20 0.0000 4 285 1605 9585 4050 many planes,\001
4 0 0 50 0 0 20 0.0000 4 285 1410 9585 4410 indexed by \001
4 0 0 50 0 0 22 0.0000 4 225 195 11025 4410 Z\001


==> figures/i1example8 <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
6 4590 4815 6390 5850
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 5175 4860 4635 5805 5805 5805
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 5805 5805 6345 4860 5175 4860
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 4950 5265 5670 5310 4905 5355
-6
6 4590 5940 6390 6975
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 5175 5985 4635 6930 5805 6930
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 5805 6930 6345 5985 5175 5985
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 4950 6390 5670 6435 4905 6480
-6
6 4815 1980 6615 3015
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 5400 2025 4860 2970 6030 2970
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 6030 2970 6570 2025 5400 2025
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 5175 2430 5895 2475 5130 2520
-6
6 4995 855 6795 1890
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 5580 900 5040 1845 6210 1845
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 6210 1845 6750 900 5580 900
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 5355 1305 6075 1350 5310 1395
-6
6 7560 4815 9360 5850
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 8145 4860 7605 5805 8775 5805
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 8775 5805 9315 4860 8145 4860
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 9090 5265 8280 5310 9045 5355
4 0 0 50 0 0 18 0.0000 4 180 135 8235 5220 1\001
-6
6 7560 5895 9360 6930
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 8145 5940 7605 6885 8775 6885
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 8775 6885 9315 5940 8145 5940
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 9090 6345 8280 6390 9045 6435
4 0 0 50 0 0 18 0.0000 4 180 135 8235 6300 1\001
-6
6 7785 855 9585 1890
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 8370 900 7830 1845 9000 1845
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 9000 1845 9540 900 8370 900
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 9315 1305 8505 1350 9270 1395
4 0 0 50 0 0 18 0.0000 4 180 135 8460 1260 1\001
-6
6 7695 2025 9495 3060
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 8280 2070 7740 3015 8910 3015
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 8910 3015 9450 2070 8280 2070
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 9225 2475 8415 2520 9180 2565
4 0 0 50 0 0 18 0.0000 4 180 135 8370 2430 1\001
-6
6 3285 3600 3510 3915
4 0 0 50 0 33 30 0.0000 4 285 210 3285 3870 S\001
-6
6 5805 270 5985 810
1 3 0 2 0 0 50 0 20 0.000 1 0.0000 5895 720 32 32 5895 720 5927 720
1 3 0 2 0 0 50 0 20 0.000 1 0.0000 5895 540 32 32 5895 540 5927 540
1 3 0 2 0 0 50 0 20 0.000 1 0.0000 5895 360 32 32 5895 360 5927 360
-6
6 5445 7020 5625 7560
1 3 0 2 0 0 50 0 20 0.000 1 0.0000 5535 7470 32 32 5535 7470 5567 7470
1 3 0 2 0 0 50 0 20 0.000 1 0.0000 5535 7290 32 32 5535 7290 5567 7290
1 3 0 2 0 0 50 0 20 0.000 1 0.0000 5535 7110 32 32 5535 7110 5567 7110
-6
6 8280 6975 8460 7515
1 3 0 2 0 0 50 0 20 0.000 1 0.0000 8370 7425 32 32 8370 7425 8402 7425
1 3 0 2 0 0 50 0 20 0.000 1 0.0000 8370 7245 32 32 8370 7245 8402 7245
1 3 0 2 0 0 50 0 20 0.000 1 0.0000 8370 7065 32 32 8370 7065 8402 7065
-6
6 8685 270 8865 810
1 3 0 2 0 0 50 0 20 0.000 1 0.0000 8775 720 32 32 8775 720 8807 720
1 3 0 2 0 0 50 0 20 0.000 1 0.0000 8775 540 32 32 8775 540 8807 540
1 3 0 2 0 0 50 0 20 0.000 1 0.0000 8775 360 32 32 8775 360 8807 360
-6
2 3 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 5
	 8820 4590 4680 4590 5400 3195 9540 3195 8820 4590
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 5130 3780 5850 3825 5085 3870
2 1 0 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 9225 3780 8415 3825 9180 3870
4 0 0 50 0 0 18 0.0000 4 180 225 5805 3735 -1\001
4 0 0 50 0 0 18 0.0000 4 180 135 8325 3735 1\001
4 0 0 50 0 0 18 0.0000 4 180 225 5625 5220 -1\001
4 0 0 50 0 0 18 0.0000 4 180 225 5580 6345 -1\001
4 0 0 50 0 0 18 0.0000 4 180 225 5850 2385 -1\001
4 0 0 50 0 0 18 0.0000 4 180 225 5940 1305 -1\001
4 0 0 50 0 0 20 0.0000 4 195 1695 1395 3915 Gauss surface\001
4 0 0 50 0 0 16 0.0000 4 165 585 3510 4050 Gauss\001


==> figures/i2fig1 <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
6 4140 2250 8415 3645
2 3 0 2 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 7470 3600 4185 3600 5085 2295 8370 2295 7470 3600
-6
6 4140 3915 8415 5310
2 3 0 2 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 7470 5265 4185 5265 5085 3960 8370 3960 7470 5265
-6
6 4590 4365 5580 4635
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 4590 4635 4590
4 0 0 50 0 0 18 0.0000 4 180 135 5445 4545 0\001
-6
6 4590 2745 5580 3015
2 1 0 2 0 0 50 0 -1 0.000 0 0 7 0 0 2
	 5400 2970 4635 2970
4 0 0 50 0 0 18 0.0000 4 180 135 5445 2925 0\001
-6
1 4 0 2 0 0 50 0 41 0.000 1 0.0000 5850 2587 68 68 5850 2520 5850 2655
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6390 2970 7920 2970
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6975 4590 7920 4590
2 1 0 2 0 0 50 0 -1 0.000 0 0 -1 0 0 2
	 5175 2745 5355 2745
2 1 0 2 0 0 50 0 -1 0.000 0 0 -1 0 0 2
	 5220 2745 5265 2610
2 1 0 2 0 0 50 0 -1 0.000 0 0 -1 0 0 2
	 5895 5085 5805 5175
2 1 0 2 0 0 50 0 -1 0.000 0 0 -1 0 0 2
	 5895 5085 5805 4995
2 1 0 2 0 0 50 0 -1 0.000 0 0 -1 0 0 2
	 6345 2655 6390 2790
2 1 0 2 0 0 50 0 -1 0.000 0 0 -1 0 0 2
	 6390 2655 6525 2610
3 0 0 2 0 0 50 0 -1 0.000 0 0 0 6
	 5850 2610 5580 2610 5265 2700 5130 2790 5085 2880 5085 2970
	 0.000 1.000 1.000 1.000 1.000 0.000
3 0 0 2 0 0 50 0 -1 0.000 0 0 0 9
	 4995 4590 4995 4815 5130 4950 5580 5085 6120 5085 6840 4995
	 7155 4905 7245 4770 7290 4590
	 0.000 1.000 1.000 1.000 1.000 1.000 1.000 1.000
	 0.000
3 0 0 2 0 0 50 0 -1 0.000 0 0 0 5
	 6705 2970 6660 2835 6525 2700 6300 2610 5850 2565
	 0.000 1.000 1.000 1.000 0.000
4 0 0 50 0 0 18 0.0000 4 180 195 6120 2970  1\001
4 0 0 50 0 0 18 0.0000 4 180 135 6750 4590 2\001


==> figures/i2fig2 <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
6 4140 3915 8415 5310
6 4140 3915 8415 5310
2 3 0 2 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 7470 5265 4185 5265 5085 3960 8370 3960 7470 5265
-6
6 4590 4365 5670 4635
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 4590 4635 4590
4 0 0 50 0 0 18 0.0000 4 180 225 5445 4545 -1\001
-6
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 4590 7920 4590
4 0 0 50 0 0 18 0.0000 4 180 135 6975 4590 1\001
-6
6 4140 2250 8415 3645
6 4140 2250 8415 3645
2 3 0 2 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 7470 3600 4185 3600 5085 2295 8370 2295 7470 3600
-6
6 4590 2700 5670 2970
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 2925 4635 2925
4 0 0 50 0 0 18 0.0000 4 180 225 5445 2880 -1\001
-6
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 2925 7920 2925
4 0 0 50 0 0 18 0.0000 4 180 135 6975 2925 1\001
-6
6 6435 1350 6615 1980
1 4 0 2 0 0 50 0 41 0.000 1 0.0000 6502 1890 40 40 6462 1890 6542 1890
1 4 0 2 0 0 50 0 41 0.000 1 0.0000 6525 1665 40 40 6485 1665 6565 1665
1 4 0 2 0 0 50 0 41 0.000 1 0.0000 6525 1440 40 40 6485 1440 6565 1440
-6
6 6435 5535 6615 6165
1 4 0 2 0 0 50 0 41 0.000 1 0.0000 6502 6075 40 40 6462 6075 6542 6075
1 4 0 2 0 0 50 0 41 0.000 1 0.0000 6525 5850 40 40 6485 5850 6565 5850
1 4 0 2 0 0 50 0 41 0.000 1 0.0000 6525 5625 40 40 6485 5625 6565 5625
-6
2 1 0 2 0 0 50 0 41 0.000 0 0 -1 0 0 2
	 6345 3960 6345 4995
2 1 0 2 0 0 50 0 41 0.000 0 0 -1 0 0 2
	 6345 2295 6345 3060
2 1 1 2 0 0 50 0 -1 6.000 0 0 7 0 0 3
	 5400 4590 6345 4995 7200 4590
2 1 1 2 0 0 50 0 -1 6.000 0 0 -1 0 0 3
	 5400 2925 6345 3060 7245 2925
4 0 0 50 0 2 20 0.0000 4 210 900 8550 4815 sheet n\001
4 0 0 50 0 2 20 0.0000 4 210 1215 8550 3150 sheet n+1\001


==> figures/i2fig3 <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
6 4140 3915 8415 5310
2 3 0 2 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 7470 5265 4185 5265 5085 3960 8370 3960 7470 5265
-6
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 2925 7920 2925
2 3 0 2 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 7470 3600 4185 3600 5085 2295 8370 2295 7470 3600
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 4590 7920 4590
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 2925 4635 2925
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 4590 4635 4590
2 1 1 2 0 0 50 0 -1 6.000 0 0 -1 0 0 2
	 5445 2925 7200 2925
2 1 1 2 0 0 50 0 -1 6.000 0 0 -1 0 0 2
	 5445 4590 7155 4590
4 0 0 50 0 0 18 0.0000 4 180 135 7020 2880 1\001
4 0 0 50 0 0 18 0.0000 4 180 135 6975 4545 1\001
4 0 0 50 0 0 18 0.0000 4 180 225 5445 2835 -1\001
4 0 0 50 0 0 18 0.0000 4 180 225 5445 4500 -1\001


==> figures/i2fig4 <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
6 2205 2160 10665 6120
6 3240 3870 7515 5265
6 3240 3870 7515 5265
2 3 0 2 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 6570 5220 3285 5220 4185 3915 7470 3915 6570 5220
-6
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6300 4545 7020 4545
-6
6 3375 2160 7650 3555
6 3375 2160 7650 3555
2 3 0 2 0 7 50 0 -1 0.000 0 0 7 0 0 5
	 6705 3510 3420 3510 4320 2205 7605 2205 6705 3510
-6
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6435 2835 7155 2835
-6
6 2205 5805 9000 6120
6 3870 5985 4005 6120
6 3870 5985 4005 6120
4 0 0 50 0 0 12 0.0000 4 120 135 3870 6120  0\001
-6
-6
4 0 0 50 0 0 22 0.0000 4 300 6780 2205 6030 A circle C(w ,r) on the surface of the square root   \001
-6
1 1 0 2 0 7 50 0 -1 0.000 1 0.0000 5625 2835 1260 450 5625 2835 4365 3285
1 1 0 2 0 7 50 0 -1 0.000 1 0.0000 6300 4545 405 225 6300 4545 6705 4770
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 1
	 5625 2835
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 1 2
	0 0 2.00 120.00 240.00
	 6930 2610 8415 2340
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 1 2
	0 0 2.00 120.00 240.00
	 6656 4296 8141 4026
4 0 0 50 0 0 20 0.0000 4 210 1635 8505 2430 Arc centered \001
4 0 0 50 0 0 20 0.0000 4 210 1125 8505 2790 around w\001
4 0 0 50 0 0 20 0.0000 4 135 210 5580 2745 w\001
4 0 0 50 0 0 12 0.0000 4 120 135 5760 2790  0\001
4 0 0 50 0 0 12 0.0000 4 120 135 9585 2880  0\001
4 0 0 50 0 0 20 0.0000 4 210 1635 8235 4095 Arc centered \001
4 0 0 50 0 0 20 0.0000 4 210 2430 8235 4455 around ramification\001
4 0 0 50 0 0 20 0.0000 4 255 630 8235 4815 point\001
-6


==> figures/i2fig5 <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
6 3825 2295 8955 3915
6 3825 2295 8955 3915
2 3 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 7785 3870 3870 3870 4995 2340 8910 2340 7785 3870
-6
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4500 3015 5490 3015
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7425 3015 8415 3015
-6
6 3825 4095 8955 5715
6 3825 4095 8955 5715
2 3 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 7785 5670 3870 5670 4995 4140 8910 4140 7785 5670
-6
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4500 4815 5490 4815
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7425 4815 8415 4815
-6
2 1 0 4 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6883 2339 5893 3869
2 1 0 2 0 7 50 0 -1 0.000 0 0 -1 0 1 2
	0 0 2.00 120.00 60.00
	 6885 2250 6885 1935
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 5445 2340 4635 2835
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 5805 2340 4275 3285
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6750 2565 4455 3870
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6480 2970 4905 3870
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6255 3375 5355 3870
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 5310 4140 4770 4455
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 5805 4140 4455 4905
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6795 4140 4095 5670
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7245 4140 4680 5670
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7650 4140 5130 5670
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 8640 4140 6210 5670
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 8730 4365 6705 5670
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 8280 4995 7200 5670
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6840 2520 7245 2340
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6570 2925 7650 2385
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6165 3825 8820 2385
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6750 3870 8505 2925
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7380 3870 8055 3510
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6165 2340 4095 3555
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 5445 3060 4005 3870
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 5715 2880 6570 2340
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7380 2835 6210 3375
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7605 2700 8325 2340
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 5445 4635 4095 5355
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 5625 4500 6255 4140
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7380 4635 5715 5670
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7560 4500 8145 4140
4 0 0 50 0 0 20 0.0000 4 270 1575 6075 1845 full geodesic\001
4 0 0 50 0 0 20 0.0000 4 270 2265 765 3735 (Algebraic surface\001
4 0 0 50 0 0 20 0.0000 4 255 1965 765 4095   z   =  w (1-w) )\001
4 0 0 50 0 0 12 0.0000 4 120 90 1080 4005 2\001
4 0 0 50 0 0 20 0.0000 4 285 5025 3105 6300            "Divides" into only one half-space\001
4 0 0 50 0 2 18 0.0000 4 180 135 5490 2970 0\001
4 0 0 50 0 2 18 0.0000 4 180 135 5490 4770 0\001
4 0 0 50 0 2 18 0.0000 4 180 135 7425 2970 1\001
4 0 0 50 0 2 18 0.0000 4 180 135 7425 4770 1\001


==> figures/i2fig6 <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
6 4095 3915 8505 5130
2 3 0 2 0 7 50 0 -1 6.000 0 0 7 0 0 5
	 7515 5085 4140 5085 5085 3960 8460 3960 7515 5085
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6345 4500 7965 4545
2 1 0 4 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6795 3960 5805 5085
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6345 4514 8010 4455
-6
6 6300 1350 6480 2160
1 3 0 2 0 0 50 0 20 6.000 1 0.0000 6390 2070 45 45 6390 2070 6390 2115
1 3 0 2 0 0 50 0 20 6.000 1 0.0000 6390 1755 45 45 6390 1755 6390 1800
1 3 0 2 0 0 50 0 20 6.000 1 0.0000 6390 1440 45 45 6390 1440 6390 1485
-6
6 6300 6615 6480 7425
1 3 0 2 0 0 50 0 20 6.000 1 0.0000 6390 7335 45 45 6390 7335 6390 7380
1 3 0 2 0 0 50 0 20 6.000 1 0.0000 6390 7020 45 45 6390 7020 6390 7065
1 3 0 2 0 0 50 0 20 6.000 1 0.0000 6390 6705 45 45 6390 6705 6390 6750
-6
6 2520 3690 2745 4005
4 0 0 50 0 33 30 0.0000 4 285 210 2520 3960 S\001
-6
6 4095 2520 8505 3735
2 3 0 2 0 7 50 0 -1 6.000 0 0 7 0 0 5
	 7515 3690 4140 3690 5085 2565 8460 2565 7515 3690
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6345 3105 7965 3150
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6345 3119 8010 3060
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6570 3150 6930 3690
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6930 3150 7290 3690
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7290 3150 7605 3600
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7650 3195 7785 3375
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6255 2565 6570 3105
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6885 3060 6570 2565
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6975 2565 7290 3060
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7605 3060 7335 2565
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7740 2565 8010 3060
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 8145 2565 8235 2790
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 5940 2565 6570 3690
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 5535 2565 6210 3690
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 5130 2565 5805 3690
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 4680 3015 5130 3690
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 4500 3240 4770 3690
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 4320 3465 4455 3690
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 4916 2783 5490 3690
-6
6 4005 5220 8415 6480
2 3 0 2 0 7 50 0 -1 6.000 0 0 7 0 0 5
	 7425 6435 4050 6435 4995 5310 8370 5310 7425 6435
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6255 5850 7875 5895
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6255 5864 7920 5805
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 5220 5310 4320 6435
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 5573 5296 4673 6421
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6051 5273 5151 6398
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6501 5273 5601 6398
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7041 5273 6141 6398
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7335 5310 6930 5805
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7589 5289 7184 5784
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7949 5289 7544 5784
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6869 5919 6464 6414
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7139 5919 6734 6414
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7499 5874 7094 6369
-6
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 5580 3960 4680 4455
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6030 3960 4275 4950
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6480 3960 4545 5085
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6570 4230 5175 5085
2 1 1 2 0 7 50 0 -1 6.000 0 0 7 0 0 2
	 7020 3960 6570 4500
2 1 1 2 0 7 50 0 -1 6.000 0 0 7 0 0 2
	 7245 3960 6795 4500
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7470 3960 7110 4455
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7740 3960 7425 4455
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 8055 3960 7740 4455
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6165 4770 6435 5085
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6345 4545 6705 5085
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 6750 4545 7110 5085
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7155 4545 7470 5085
2 1 1 2 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 7515 4590 7695 4860
2 1 0 2 0 7 50 0 -1 6.000 0 0 -1 0 1 2
	0 0 2.00 120.00 60.00
	 6705 4185 8775 3465
4 0 0 50 0 0 20 0.0000 4 270 1815 1125 3600 (Surface of the\001
4 0 0 50 0 0 20 0.0000 4 270 1425 1125 3960 logarithm,  \001
4 0 0 50 0 0 16 0.0000 4 225 300 2745 4095 log\001
4 0 0 50 0 0 20 0.0000 4 255 105 3105 3915 )\001
4 0 0 50 0 0 20 0.0000 4 210 1500 1080 4725 Divides into\001
4 0 0 50 0 0 20 0.0000 4 270 2145 1080 5085 three half-spaces.\001
4 0 0 50 0 0 20 0.0000 4 270 1575 8865 3555 full geodesic\001


==> figures/i4fig2 <==
#FIG 3.2
Portrait
Center
Metric
A4 
100.0
Single
-2
1200 2
4 0 0 100 1 0 16.0 0.0 4 320.0 112.0 8640 11160 1\001
4 0 0 100 1 0 22.0 0.0 4 432.0 144.0 8460 11070 z\001
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 10530 25 25 8525 10505 8575 10555
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 1980 25 25 8525 1955 8575 2005
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 2070 25 25 8525 2045 8575 2095
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 2160 25 25 8525 2135 8575 2185
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 2250 25 25 8525 2225 8575 2275
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 2340 25 25 8525 2315 8575 2365
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 2430 25 25 8525 2405 8575 2455
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 2520 25 25 8525 2495 8575 2545
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 2700 25 25 8525 2675 8575 2725
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 2880 25 25 8525 2855 8575 2905
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 2970 25 25 8525 2945 8575 2995
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 3060 25 25 8525 3035 8575 3085
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 3150 25 25 8525 3125 8575 3175
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 3240 25 25 8525 3215 8575 3265
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 3330 25 25 8525 3305 8575 3355
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 3420 25 25 8525 3395 8575 3445
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 3600 25 25 8525 3575 8575 3625
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 3780 25 25 8525 3755 8575 3805
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 3870 25 25 8525 3845 8575 3895
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 3960 25 25 8525 3935 8575 3985
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 4050 25 25 8525 4025 8575 4075
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 4140 25 25 8525 4115 8575 4165
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 4230 25 25 8525 4205 8575 4255
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 4320 25 25 8525 4295 8575 4345
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 4500 25 25 8525 4475 8575 4525
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 4680 25 25 8525 4655 8575 4705
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 4770 25 25 8525 4745 8575 4795
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 4860 25 25 8525 4835 8575 4885
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 4950 25 25 8525 4925 8575 4975
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 5040 25 25 8525 5015 8575 5065
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 5130 25 25 8525 5105 8575 5155
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 5220 25 25 8525 5195 8575 5245
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 5220 25 25 8525 5195 8575 5245
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 5400 25 25 8525 5375 8575 5425
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 5580 25 25 8525 5555 8575 5605
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 5670 25 25 8525 5645 8575 5695
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 5760 25 25 8525 5735 8575 5785
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 5850 25 25 8525 5825 8575 5875
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 5940 25 25 8525 5915 8575 5965
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 6030 25 25 8525 6005 8575 6055
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 6120 25 25 8525 6095 8575 6145
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 6300 25 25 8525 6275 8575 6325
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 6480 25 25 8525 6455 8575 6505
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 6570 25 25 8525 6545 8575 6595
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 6660 25 25 8525 6635 8575 6685
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 6750 25 25 8525 6725 8575 6775
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 6840 25 25 8525 6815 8575 6865
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 6930 25 25 8525 6905 8575 6955
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 7020 25 25 8525 6995 8575 7045
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 7200 25 25 8525 7175 8575 7225
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 7380 25 25 8525 7355 8575 7405
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 7470 25 25 8525 7445 8575 7495
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 7470 25 25 8525 7445 8575 7495
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 7560 25 25 8525 7535 8575 7585
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 7650 25 25 8525 7625 8575 7675
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 7740 25 25 8525 7715 8575 7765
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 7830 25 25 8525 7805 8575 7855
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 7920 25 25 8525 7895 8575 7945
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 8100 25 25 8525 8075 8575 8125
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 8280 25 25 8525 8255 8575 8305
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 8370 25 25 8525 8345 8575 8395
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 8640 25 25 8525 8615 8575 8665
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 8460 25 25 8525 8435 8575 8485
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 8550 25 25 8525 8525 8575 8575
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 8730 25 25 8525 8705 8575 8755
1 1 0 1 0 0 100 1 20  6.40 1 0.0 8550 8820 25 25 8525 8795 8575 8845
4 0 0 100 1 32 22.0 0.0 4 432.0 176.0 8820 9810 p\001
2 1 0 1 0 0 100 1 -1  6.40 0 0 12 1 0 2
  0 0 1.0 144.00 240.00
       8550 9270 8550 10170
6 8820 8640 8370 8820
6 8820 8640 8370 8730
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 8730 8384 8664 8438 8640
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 8640 8820 8640
-6
6 8820 8730 8370 8820
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 8820 8820 8820
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 8730 8384 8795 8438 8820
       0.0000 1.0000 0.0000
-6
-6
6 8820 8280 8370 8460
6 8820 8370 8370 8460
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 8370 8384 8435 8438 8460
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 8460 8820 8460
-6
6 8820 8280 8370 8370
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 8280 8820 8280
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 8370 8384 8304 8438 8280
       0.0000 1.0000 0.0000
-6
-6
6 8820 7740 8370 7920
6 8820 7740 8370 7830
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 7830 8384 7764 8438 7740
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 7740 8820 7740
-6
6 8820 7830 8370 7920
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 7920 8820 7920
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 7830 8384 7895 8438 7920
       0.0000 1.0000 0.0000
-6
-6
6 8820 7380 8370 7560
6 8820 7470 8370 7560
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 7470 8384 7535 8438 7560
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 7560 8820 7560
-6
6 8820 7380 8370 7470
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 7380 8820 7380
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 7470 8384 7404 8438 7380
       0.0000 1.0000 0.0000
-6
-6
6 8820 6840 8370 7020
6 8820 6840 8370 6930
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 6930 8384 6864 8438 6840
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 6840 8820 6840
-6
6 8820 6930 8370 7020
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 7020 8820 7020
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 6930 8384 6995 8438 7020
       0.0000 1.0000 0.0000
-6
-6
6 8820 6480 8370 6660
6 8820 6570 8370 6660
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 6570 8384 6635 8438 6660
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 6660 8820 6660
-6
6 8820 6480 8370 6570
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 6480 8820 6480
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 6570 8384 6504 8438 6480
       0.0000 1.0000 0.0000
-6
-6
6 8820 5940 8370 6120
6 8820 5940 8370 6030
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 6030 8384 5964 8438 5940
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 5940 8820 5940
-6
6 8820 6030 8370 6120
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 6120 8820 6120
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 6030 8384 6095 8438 6120
       0.0000 1.0000 0.0000
-6
-6
6 8820 5580 8370 5760
6 8820 5670 8370 5760
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 5670 8384 5735 8438 5760
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 5760 8820 5760
-6
6 8820 5580 8370 5670
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 5580 8820 5580
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 5670 8384 5604 8438 5580
       0.0000 1.0000 0.0000
-6
-6
6 8820 5040 8370 5220
6 8820 5040 8370 5130
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 5130 8384 5064 8438 5040
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 5040 8820 5040
-6
6 8820 5130 8370 5220
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 5220 8820 5220
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 5130 8384 5195 8438 5220
       0.0000 1.0000 0.0000
-6
-6
6 8820 4680 8370 4860
6 8820 4770 8370 4860
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 4770 8384 4835 8438 4860
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 4860 8820 4860
-6
6 8820 4680 8370 4770
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 4680 8820 4680
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 4770 8384 4704 8438 4680
       0.0000 1.0000 0.0000
-6
-6
6 8820 4140 8370 4320
6 8820 4140 8370 4230
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 4230 8384 4164 8438 4140
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 4140 8820 4140
-6
6 8820 4230 8370 4320
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 4320 8820 4320
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 4230 8384 4295 8438 4320
       0.0000 1.0000 0.0000
-6
-6
6 8820 3780 8370 3960
6 8820 3870 8370 3960
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 3870 8384 3935 8438 3960
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 3960 8820 3960
-6
6 8820 3780 8370 3870
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 3780 8820 3780
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 3870 8384 3804 8438 3780
       0.0000 1.0000 0.0000
-6
-6
6 8820 3240 8370 3420
6 8820 3240 8370 3330
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 3330 8384 3264 8438 3240
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 3240 8820 3240
-6
6 8820 3330 8370 3420
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 3420 8820 3420
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 3330 8384 3395 8438 3420
       0.0000 1.0000 0.0000
-6
-6
6 8820 2880 8370 3060
6 8820 2970 8370 3060
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 2970 8384 3035 8438 3060
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 3060 8820 3060
-6
6 8820 2880 8370 2970
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 2880 8820 2880
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 2970 8384 2904 8438 2880
       0.0000 1.0000 0.0000
-6
-6
6 8820 2340 8370 2520
6 8820 2340 8370 2430
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 2430 8384 2364 8438 2340
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 2340 8820 2340
-6
6 8820 2430 8370 2520
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 2520 8820 2520
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 2430 8384 2495 8438 2520
       0.0000 1.0000 0.0000
-6
-6
6 8820 1980 8370 2160
6 8820 2070 8370 2160
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 2070 8384 2135 8438 2160
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 2160 8820 2160
-6
6 8820 1980 8370 2070
2 1 0 1 0 0 100 1 -1  0.32 0 0 12 0 0 2
       8438 1980 8820 1980
3 0 0 1 0 0 100 1 -1  0.32 0 0 0 3
       8370 2070 8384 2004 8438 1980
       0.0000 1.0000 0.0000
-6
-6
6 9990 8370 8100 8730
6 9990 8370 8100 8550
3 0 0 1 0 0 100 1 -1  1.36 0 0 0 3
       8100 8550 8158 8418 8387 8370
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  1.36 0 0 12 0 0 2
       8387 8370 9990 8370
-6
6 9990 8550 8100 8730
2 1 0 1 0 0 100 1 -1  1.36 0 0 12 0 0 2
       8387 8730 9990 8730
3 0 0 1 0 0 100 1 -1  1.36 0 0 0 3
       8100 8550 8158 8681 8387 8730
       0.0000 1.0000 0.0000
-6
-6
6 9990 7470 8100 7830
6 9990 7650 8100 7830
3 0 0 1 0 0 100 1 -1  1.36 0 0 0 3
       8100 7650 8158 7781 8387 7830
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  1.36 0 0 12 0 0 2
       8387 7830 9990 7830
-6
6 9990 7470 8100 7650
2 1 0 1 0 0 100 1 -1  1.36 0 0 12 0 0 2
       8387 7470 9990 7470
3 0 0 1 0 0 100 1 -1  1.36 0 0 0 3
       8100 7650 8158 7518 8387 7470
       0.0000 1.0000 0.0000
-6
-6
6 9990 6570 8100 6930
6 9990 6570 8100 6750
3 0 0 1 0 0 100 1 -1  1.36 0 0 0 3
       8100 6750 8158 6618 8387 6570
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  1.36 0 0 12 0 0 2
       8387 6570 9990 6570
-6
6 9990 6750 8100 6930
2 1 0 1 0 0 100 1 -1  1.36 0 0 12 0 0 2
       8387 6930 9990 6930
3 0 0 1 0 0 100 1 -1  1.36 0 0 0 3
       8100 6750 8158 6881 8387 6930
       0.0000 1.0000 0.0000
-6
-6
6 9990 5670 8100 6030
6 9990 5850 8100 6030
3 0 0 1 0 0 100 1 -1  1.36 0 0 0 3
       8100 5850 8158 5981 8387 6030
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  1.36 0 0 12 0 0 2
       8387 6030 9990 6030
-6
6 9990 5670 8100 5850
2 1 0 1 0 0 100 1 -1  1.36 0 0 12 0 0 2
       8387 5670 9990 5670
3 0 0 1 0 0 100 1 -1  1.36 0 0 0 3
       8100 5850 8158 5718 8387 5670
       0.0000 1.0000 0.0000
-6
-6
6 9990 4770 8100 5130
6 9990 4770 8100 4950
3 0 0 1 0 0 100 1 -1  1.36 0 0 0 3
       8100 4950 8158 4818 8387 4770
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  1.36 0 0 12 0 0 2
       8387 4770 9990 4770
-6
6 9990 4950 8100 5130
2 1 0 1 0 0 100 1 -1  1.36 0 0 12 0 0 2
       8387 5130 9990 5130
3 0 0 1 0 0 100 1 -1  1.36 0 0 0 3
       8100 4950 8158 5081 8387 5130
       0.0000 1.0000 0.0000
-6
-6
6 9990 3870 8100 4230
6 9990 4050 8100 4230
3 0 0 1 0 0 100 1 -1  1.36 0 0 0 3
       8100 4050 8158 4181 8387 4230
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  1.36 0 0 12 0 0 2
       8387 4230 9990 4230
-6
6 9990 3870 8100 4050
2 1 0 1 0 0 100 1 -1  1.36 0 0 12 0 0 2
       8387 3870 9990 3870
3 0 0 1 0 0 100 1 -1  1.36 0 0 0 3
       8100 4050 8158 3918 8387 3870
       0.0000 1.0000 0.0000
-6
-6
6 9990 2970 8100 3330
6 9990 2970 8100 3150
3 0 0 1 0 0 100 1 -1  1.36 0 0 0 3
       8100 3150 8158 3018 8387 2970
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  1.36 0 0 12 0 0 2
       8387 2970 9990 2970
-6
6 9990 3150 8100 3330
2 1 0 1 0 0 100 1 -1  1.36 0 0 12 0 0 2
       8387 3330 9990 3330
3 0 0 1 0 0 100 1 -1  1.36 0 0 0 3
       8100 3150 8158 3281 8387 3330
       0.0000 1.0000 0.0000
-6
-6
6 9990 2070 8100 2430
6 9990 2250 8100 2430
3 0 0 1 0 0 100 1 -1  1.36 0 0 0 3
       8100 2250 8158 2381 8387 2430
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  1.36 0 0 12 0 0 2
       8387 2430 9990 2430
-6
6 9990 2070 8100 2250
2 1 0 1 0 0 100 1 -1  1.36 0 0 12 0 0 2
       8387 2070 9990 2070
3 0 0 1 0 0 100 1 -1  1.36 0 0 0 3
       8100 2250 8158 2118 8387 2070
       0.0000 1.0000 0.0000
-6
-6
6 11160 2250 6930 3150
6 11160 2250 6930 2700
3 0 0 1 0 0 100 1 -1  3.04 0 0 0 3
       6930 2700 7059 2370 7571 2250
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  3.04 0 0 12 0 0 2
       7571 2250 11160 2250
-6
6 11160 2700 6930 3150
2 1 0 1 0 0 100 1 -1  3.04 0 0 12 0 0 2
       7571 3150 11160 3150
3 0 0 1 0 0 100 1 -1  3.04 0 0 0 3
       6930 2700 7059 3029 7571 3150
       0.0000 1.0000 0.0000
-6
-6
6 11160 7650 6930 8550
6 11160 7650 6930 8100
3 0 0 1 0 0 100 1 -1  3.04 0 0 0 3
       6930 8100 7059 7770 7571 7650
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  3.04 0 0 12 0 0 2
       7571 7650 11160 7650
-6
6 11160 8100 6930 8550
2 1 0 1 0 0 100 1 -1  3.04 0 0 12 0 0 2
       7571 8550 11160 8550
3 0 0 1 0 0 100 1 -1  3.04 0 0 0 3
       6930 8100 7059 8429 7571 8550
       0.0000 1.0000 0.0000
-6
-6
6 11160 5850 6930 6750
6 11160 6300 6930 6750
3 0 0 1 0 0 100 1 -1  3.04 0 0 0 3
       6930 6300 7059 6629 7571 6750
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  3.04 0 0 12 0 0 2
       7571 6750 11160 6750
-6
6 11160 5850 6930 6300
2 1 0 1 0 0 100 1 -1  3.04 0 0 12 0 0 2
       7571 5850 11160 5850
3 0 0 1 0 0 100 1 -1  3.04 0 0 0 3
       6930 6300 7059 5970 7571 5850
       0.0000 1.0000 0.0000
-6
-6
6 11160 4050 6930 4950
6 11160 4050 6930 4500
3 0 0 1 0 0 100 1 -1  3.04 0 0 0 3
       6930 4500 7059 4170 7571 4050
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  3.04 0 0 12 0 0 2
       7571 4050 11160 4050
-6
6 11160 4500 6930 4950
2 1 0 1 0 0 100 1 -1  3.04 0 0 12 0 0 2
       7571 4950 11160 4950
3 0 0 1 0 0 100 1 -1  3.04 0 0 0 3
       6930 4500 7059 4829 7571 4950
       0.0000 1.0000 0.0000
-6
-6
6 11160 2250 6930 3150
6 11160 2700 6930 3150
3 0 0 1 0 0 100 1 -1  3.04 0 0 0 3
       6930 2700 7059 3029 7571 3150
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  3.04 0 0 12 0 0 2
       7571 3150 11160 3150
-6
6 11160 2250 6930 2700
2 1 0 1 0 0 100 1 -1  3.04 0 0 12 0 0 2
       7571 2250 11160 2250
3 0 0 1 0 0 100 1 -1  3.04 0 0 0 3
       6930 2700 7059 2370 7571 2250
       0.0000 1.0000 0.0000
-6
-6
2 1 0 1 0 0 100 1 -1  6.40 0 0 12 0 0 2
       450 10530 11160 10530
6 11160 6300 4230 8100
6 11160 7200 4230 8100
3 0 0 1 0 0 100 1 -1  4.98 0 0 0 3
       4230 7200 4440 7860 5280 8100
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  4.98 0 0 12 0 0 2
       5280 8100 11160 8100
-6
6 11160 6300 4230 7200
2 1 0 1 0 0 100 1 -1  4.98 0 0 12 0 0 2
       5280 6300 11160 6300
3 0 0 1 0 0 100 1 -1  4.98 0 0 0 3
       4230 7200 4440 6540 5280 6300
       0.0000 1.0000 0.0000
-6
-6
6 11160 2700 4230 4500
6 11160 2700 4230 3600
3 0 0 1 0 0 100 1 -1  4.98 0 0 0 3
       4230 3600 4440 2940 5280 2700
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  4.98 0 0 12 0 0 2
       5280 2700 11160 2700
-6
6 11160 3600 4230 4500
2 1 0 1 0 0 100 1 -1  4.98 0 0 12 0 0 2
       5280 4500 11160 4500
3 0 0 1 0 0 100 1 -1  4.98 0 0 0 3
       4230 3600 4440 4260 5280 4500
       0.0000 1.0000 0.0000
-6
-6
6 11160 3600 2250 7200
6 11160 5400 2250 7200
3 0 0 1 0 0 100 1 -1  6.40 0 0 0 3
       2250 5400 2520 6720 3600 7200
       0.0000 1.0000 0.0000
2 1 0 1 0 0 100 1 -1  6.40 0 0 12 0 0 2
       3600 7200 11160 7200
-6
6 11160 3600 2250 5400
2 1 0 1 0 0 100 1 -1  6.40 0 0 12 0 0 2
       3600 3600 11160 3600
3 0 0 1 0 0 100 1 -1  6.40 0 0 0 3
       2250 5400 2520 4080 3600 3600
       0.0000 1.0000 0.0000
-6
-6
2 1 0 1 0 0 100 1 -1  6.40 0 0 12 0 0 2
       450 5400 11160 5400

